Securing DRAM at Scale: ARFM-Driven Row Hammer Defense with Unveiling the Threat of Short tRC Patterns

To address the issue of powerful row hammer (RH) attacks, our study involved an extensive analysis of the prevalent attack patterns in the field. We discovered a strong correlation between the timing and density of the active-to-active command period, ${tRC}$, and the likelihood of RH attacks. In this paper, we introduce MARC, an innovative ARFM-driven RH mitigation IP that significantly reinforces existing RH mitigation IPs. MARC dynamically adjusts the frequency of RFM in response to the severity of the RH attack environment, offering a tailored security solution that not only detects the threats but also adapts to varying threat levels. MARC's detection mechanism has demonstrated remarkable efficiency, identifying over 99\% of attack patterns. Moreover, MARC is designed as a compact hardware module, facilitating tight integration either on the memory controller-side or DRAM-side within the memory system. It only occupies a negligible hardware area of 3363~\textit{$\mu m^2$}. By activating ARFM based on MARC's detection, the additional energy overhead is also negligible in normal workloads. We conduct experiments to compare the highest row count throughout the patterns, defined as max exposure, between the vanilla RH mitigation IPs and the MARC-enhanced versions of the same IPs, focusing on both DRAM-side and memory controller-side. On the DRAM-side, MARC + probabilistic scheme and MARC + counter-based tracking scheme achieve 8.1$\times$ and 1.5$\times$ improvement in max exposure ratio compared to the vanilla IPs, respectively. On the memory controller-side, the MARC + PARA and MARC + Graphene achieve 50$\times$ and 5.7$\times$ improvement in max exposure ratio compared to the vanilla IPs, respectively. MARC ensures optimal security without sacrificing system performance, making MARC a pioneering solution in the realm of RH attack mitigation.

==> arxiv/ref.tex <==
@book{lamport94,
 author = "Leslie Lamport",
 title = "{\LaTeX: A Document Preparation System}",
 year = "1994",
 publisher = "Addison-Wesley",
 edition = "2nd",
 address = "Reading, Massachusetts"
}

@inproceedings{nicepaper1,
  author = "Firstname1 Lastname1 and Firstname2 Lastname2",
  title = "A Very Nice Paper To Cite",
  year = "2016",
  booktitle = "Proceedings of the 49th Annual IEEE/ACM International Symposium on Microarchitecture"
}

@inproceedings{nicepaper2,
  author = "Firstname1 Lastname1 and Firstname2 Lastname2 and Firstname3 Lastname3",
  title = "Another Very Nice Paper to Cite",
  year = "2015",
  booktitle = "Proceedings of the 48th Annual IEEE/ACM International Symposium on Microarchitecture"
}

@inproceedings{nicepaper3,
  author = "Firstname1 Lastname1 and Firstname2 Lastname2 and Firstname3 Lastname3 and Firstname4 Lastname4 and Firstname5 Lastname5 and Firstname6 Lastname6 and Firstname7 Lastname7 and Firstname8 Lastname8 and Firstname9 Lastname9 and Firstname10 Lastname10 and Firstname11 Lastname11 and Firstname12 Lastname12",
  title = "Yet Another Very Nice Paper To Cite, With Many Author Names All Spelled Out",
  year = "2011",
  booktitle = "Proceedings of the 38th Annual International Symposium on Computer Architecture"
}

@article{kim2014flipping,
  title={Flipping bits in memory without accessing them: An experimental study of DRAM disturbance errors},
  author={Kim, Yoongu and Daly, Ross and Kim, Jeremie and Fallin, Chris and Lee, Ji Hye and Lee, Donghyuk and Wilkerson, Chris and Lai, Konrad and Mutlu, Onur},
  journal={ACM SIGARCH Computer Architecture News},
  volume={42},
  number={3},
  pages={361--372},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@article{cha2011dram,
  title={DRAM and future commodity memories},
  author={Cha, SY},
  journal={VLSI Technology Short Course},
  year={2011}
}

@article{mandelman2002challenges,
  title={Challenges and future directions for the scaling of dynamic random-access memory (DRAM)},
  author={Mandelman, Jack A and Dennard, Robert H and Bronner, Gary B and DeBrosse, John K and Divakaruni, Rama and Li, Yujun and Radens, Carl J},
  journal={IBM Journal of Research and Development},
  volume={46},
  number={2.3},
  pages={187--212},
  year={2002},
  publisher={IBM}
}

@article{yoon2013flash,
  title={Flash \& DRAM Si scaling challenges, emerging non-volatile memory technology enablement--implications to enterprise storage and server compute systems},
  author={Yoon, Jung H and Hunter, Hillery C and Tressler, Gary A},
  journal={Flash Memory Summit},
  year={2013}
}

@article{konishi1989analysis,
  title={Analysis of coupling noise between adjacent bit lines in megabit DRAMs},
  author={Konishi, Yasuhiro and Kumanoya, Masaki and Yamasaki, Hiroyuki and Dosaka, Katsumi and Yoshihara, Tsutomu},
  journal={IEEE Journal of Solid-State Circuits},
  volume={24},
  number={1},
  pages={35--42},
  year={1989},
  publisher={IEEE}
}

@inproceedings{redeker2002investigation,
  title={An investigation into crosstalk noise in DRAM structures},
  author={Redeker, Michael and Cockburn, Bruce F and Elliott, Duncan G},
  booktitle={Proceedings of the 2002 IEEE International Workshop on Memory Technology, Design and Testing (MTDT2002)},
  pages={123--129},
  year={2002},
  organization={IEEE}
}

@inproceedings{mutlu2017rowhammer,
  title={The RowHammer problem and other issues we may face as memory becomes denser},
  author={Mutlu, Onur},
  booktitle={Design, Automation \& Test in Europe Conference \& Exhibition (DATE), 2017},
  pages={1116--1121},
  year={2017},
  organization={IEEE}
}

@article{chang2017understanding,
  title={Understanding reduced-voltage operation in modern DRAM devices: Experimental characterization, analysis, and mechanisms},
  author={Chang, Kevin K and Ya{\u{g}}l{\i}k{\c{c}}{\i}, A Giray and Ghose, Saugata and Agrawal, Aditya and Chatterjee, Niladrish and Kashyap, Abhijith and Lee, Donghyuk and O'Connor, Mike and Hassan, Hasan and Mutlu, Onur},
  journal={Proceedings of the ACM on Measurement and Analysis of Computing Systems},
  volume={1},
  number={1},
  pages={1--42},
  year={2017},
  publisher={ACM New York, NY, USA}
}

@inproceedings{chang2016understanding,
  title={Understanding latency variation in modern DRAM chips: Experimental characterization, analysis, and optimization},
  author={Chang, Kevin K and Kashyap, Abhijith and Hassan, Hasan and Ghose, Saugata and Hsieh, Kevin and Lee, Donghyuk and Li, Tianshi and Pekhimenko, Gennady and Khan, Samira and Mutlu, Onur},
  booktitle={Proceedings of the 2016 ACM SIGMETRICS International Conference on Measurement and Modeling of Computer Science},
  pages={323--336},
  year={2016}
}

@inproceedings{park2020graphene,
  title={Graphene: Strong yet lightweight row hammer protection},
  author={Park, Yeonhong and Kwon, Woosuk and Lee, Eojin and Ham, Tae Jun and Ahn, Jung Ho and Lee, Jae W},
  booktitle={2020 53rd Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={1--13},
  year={2020},
  organization={IEEE}
}

@inproceedings{kim2022mithril,
  title={Mithril: Cooperative row hammer protection on commodity dram leveraging managed refresh},
  author={Kim, Michael Jaemin and Park, Jaehyun and Park, Yeonhong and Doh, Wanju and Kim, Namhoon and Ham, Tae Jun and Lee, Jae W and Ahn, Jung Ho},
  booktitle={2022 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={1156--1169},
  year={2022},
  organization={IEEE}
}

@inproceedings{lee2019twice,
  title={TWiCe: Preventing row-hammering by exploiting time window counters},
  author={Lee, Eojin and Kang, Ingab and Lee, Sukhan and Suh, G Edward and Ahn, Jung Ho},
  booktitle={Proceedings of the 46th International Symposium on Computer Architecture},
  pages={385--396},
  year={2019}
}

@inproceedings{yauglikcci2021blockhammer,
  title={Blockhammer: Preventing rowhammer at low cost by blacklisting rapidly-accessed dram rows},
  author={Ya{\u{g}}lik{\c{c}}i, A Giray and Patel, Minesh and Kim, Jeremie S and Azizi, Roknoddin and Olgun, Ataberk and Orosa, Lois and Hassan, Hasan and Park, Jisung and Kanellopoulos, Konstantinos and Shahroodi, Taha and others},
  booktitle={2021 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={345--358},
  year={2021},
  organization={IEEE}
}

@inproceedings{frigo2020trrespass,
  title={TRRespass: Exploiting the many sides of target row refresh},
  author={Frigo, Pietro and Vannacc, Emanuele and Hassan, Hasan and Van Der Veen, Victor and Mutlu, Onur and Giuffrida, Cristiano and Bos, Herbert and Razavi, Kaveh},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={747--762},
  year={2020},
  organization={IEEE}
}

@inproceedings{aga2017good,
  title={When good protections go bad: Exploiting anti-DoS measures to accelerate Rowhammer attacks},
  author={Aga, Misiker Tadesse and Aweke, Zelalem Birhanu and Austin, Todd},
  booktitle={2017 IEEE International Symposium on Hardware Oriented Security and Trust (HOST)},
  pages={8--13},
  year={2017},
  organization={IEEE}
}

@inproceedings{gruss2018another,
  title={Another flip in the wall of rowhammer defenses},
  author={Gruss, Daniel and Lipp, Moritz and Schwarz, Michael and Genkin, Daniel and Juffinger, Jonas and O'Connell, Sioli and Schoechl, Wolfgang and Yarom, Yuval},
  booktitle={2018 IEEE Symposium on Security and Privacy (SP)},
  pages={245--261},
  year={2018},
  organization={IEEE}
}

@inproceedings{jattke2022blacksmith,
  title={Blacksmith: Scalable rowhammering in the frequency domain},
  author={Jattke, Patrick and Van Der Veen, Victor and Frigo, Pietro and Gunter, Stijn and Razavi, Kaveh},
  booktitle={2022 IEEE Symposium on Security and Privacy (SP)},
  pages={716--734},
  year={2022},
  organization={IEEE}
}

@inproceedings{van2018guardion,
  title={Guardion: Practical mitigation of dma-based rowhammer attacks on arm},
  author={Van der Veen, Victor and Lindorfer, Martina and Fratantonio, Yanick and Padmanabha Pillai, Harikrishnan and Vigna, Giovanni and Kruegel, Christopher and Bos, Herbert and Razavi, Kaveh},
  booktitle={Detection of Intrusions and Malware, and Vulnerability Assessment: 15th International Conference, DIMVA 2018, Saclay, France, June 28--29, 2018, Proceedings 15},
  pages={92--113},
  year={2018},
  organization={Springer}
}

@article{aweke2016anvil,
  title={ANVIL: Software-based protection against next-generation rowhammer attacks},
  author={Aweke, Zelalem Birhanu and Yitbarek, Salessawi Ferede and Qiao, Rui and Das, Reetuparna and Hicks, Matthew and Oren, Yossi and Austin, Todd},
  journal={ACM SIGPLAN Notices},
  volume={51},
  number={4},
  pages={743--755},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@inproceedings{son2017making,
  title={Making DRAM stronger against row hammering},
  author={Son, Mungyu and Park, Hyunsun and Ahn, Junwhan and Yoo, Sungjoo},
  booktitle={Proceedings of the 54th Annual Design Automation Conference 2017},
  pages={1--6},
  year={2017}
}

@inproceedings{you2019mrloc,
  title={MRLoc: Mitigating Row-hammering based on memory Locality},
  author={You, Jung Min and Yang, Joon-Sung},
  booktitle={Proceedings of the 56th Annual Design Automation Conference 2019},
  pages={1--6},
  year={2019}
}

@inproceedings{marazzi2022protrr,
  title={Protrr: Principled yet optimal in-dram target row refresh},
  author={Marazzi, Michele and Jattke, Patrick and Solt, Flavien and Razavi, Kaveh},
  booktitle={2022 IEEE Symposium on Security and Privacy (SP)},
  pages={735--753},
  year={2022},
  organization={IEEE}
}

@inproceedings{kim20231,
  title={A 1.1 V 16Gb DDR5 DRAM with Probabilistic-Aggressor Tracking, Refresh-Management Functionality, Per-Row Hammer Tracking, a Multi-Step Precharge, and Core-Bias Modulation for Security and Reliability Enhancement},
  author={Kim, Woongrae and Jung, Chulmoon and Yoo, Seongnyuh and Hong, Duckhwa and Hwang, Jeongjin and Yoon, Jungmin and Jung, Ohyong and Choi, Joonwoo and Hyun, Sanga and Kang, Mankeun and others},
  booktitle={2023 IEEE International Solid-State Circuits Conference (ISSCC)},
  pages={1--3},
  year={2023},
  organization={IEEE}
}

@inproceedings{orosa2021deeper,
  title={A deeper look into rowhammer’s sensitivities: Experimental analysis of real dram chips and implications on future attacks and defenses},
  author={Orosa, Lois and Yaglikci, Abdullah Giray and Luo, Haocong and Olgun, Ataberk and Park, Jisung and Hassan, Hasan and Patel, Minesh and Kim, Jeremie S and Mutlu, Onur},
  booktitle={MICRO-54: 54th Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={1182--1197},
  year={2021}
}

@inproceedings{cojocar2019exploiting,
  title={Exploiting correcting codes
         : On the effectiveness of ecc memory against rowhammer attacks},
  author={Cojocar, Lucian and Razavi, Kaveh and Giuffrida, Cristiano and Bos, Herbert},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={55--71},
  year={2019},
  organization={IEEE}
}

@inproceedings{gruss2016rowhammer,
  title={Rowhammer. js: A remote software-induced fault attack in javascript},
  author={Gruss, Daniel and Maurice, Cl{\'e}mentine and Mangard, Stefan},
  booktitle={Detection of Intrusions and Malware, and Vulnerability Assessment: 13th International Conference, DIMVA 2016, San Sebasti{\'a}n, Spain, July 7-8, 2016, Proceedings 13},
  pages={300--321},
  year={2016},
  organization={Springer}
}

@article{kim2014architectural,
  title={Architectural support for mitigating row hammering in DRAM memories},
  author={Kim, Dae-Hyun and Nair, Prashant J and Qureshi, Moinuddin K},
  journal={IEEE Computer Architecture Letters},
  volume={14},
  number={1},
  pages={9--12},
  year={2014},
  publisher={IEEE}
}

@article{seyedzadeh2016counter,
  title={Counter-based tree structure for row hammering mitigation in DRAM},
  author={Seyedzadeh, Seyed Mohammad and Jones, Alex K and Melhem, Rami},
  journal={IEEE Computer Architecture Letters},
  volume={16},
  number={1},
  pages={18--21},
  year={2016},
  publisher={IEEE}
}

@article{kim2015ramulator,
  title={Ramulator: A fast and extensible DRAM simulator},
  author={Kim, Yoongu and Yang, Weikun and Mutlu, Onur},
  journal={IEEE Computer architecture letters},
  volume={15},
  number={1},
  pages={45--49},
  year={2015},
  publisher={IEEE}
}



@book{jedeclpddr5,
    author = {JEDEC},
    title = {LPDDR5 Standard JESD209-5},
        year = {2019} 
}

@book{jedecddr5,
    author = {JEDEC},
    title = {DDR5 SDRAM},
        year = {2020} 
}
